Ming-Omni: A Unified Multimodal Model for Perception and Generation

We propose Ming-Omni, a unified multimodal model capable of processing images, text, audio, and video, while demonstrating strong proficiency in both speech and image generation. Ming-Omni employs dedicated encoders to extract tokens from different modalities, which are then processed by Ling, an MoE architecture equipped with newly proposed modality-specific routers. This design enables a single model to efficiently process and fuse multimodal inputs within a unified framework, thereby facilitating diverse tasks without requiring separate models, task-specific fine-tuning, or structural redesign. Importantly, Ming-Omni extends beyond conventional multimodal models by supporting audio and image generation. This is achieved through the integration of an advanced audio decoder for natural-sounding speech and Ming-Lite-Uni for high-quality image generation, which also allow the model to engage in context-aware chatting, perform text-to-speech conversion, and conduct versatile image editing. Our experimental results showcase Ming-Omni offers a powerful solution for unified perception and generation across all modalities. Notably, our proposed Ming-Omni is the first open-source model we are aware of to match GPT-4o in modality support, and we release all code and model weights to encourage further research and development in the community.

==> readme.tex <==
# Antu-α: Unified Visual Understanding & Generation Framework
paper: [url](url)
## Core Technical Breakthroughs

- ### Unified Visual Understanding & Generation Architecture
	Introduces a shared representation space for vision-language tasks, replacing traditional CLIP+Diffusion pipelines. The architecture leverages **learnable multiscale-queries** that dynamically integrate multimodal signals, enabling seamless end-to-end sequence prediction for text→image→editing workflows. This approach effectively addresses the quality limitations of discrete token-based methods. Our Antu-α achieves the unification of generation and understanding, with an average understanding score of 69.7 on the OpenCompass leaderboard, surpassing DeepSeek-VL2 (66.4). At the same time, it maintains strong generation capabilities, achieving a generation score of 61.9 on the GenEval benchmark, outperforming SDXL (0.55).


- ### Multi-Scale Learnable Query Token
	Employs a novel mechanism to establish feature correlations across resolutions of 4×/8×/16×. By introducing **hierarchical tokens**, the model resolves cross-scale inconsistencies in super-resolution and editing tasks. 

- ### Cross-Scale Consistency Loss
  A **cross-scale consistency loss** is applied, leveraging explicit gradient constraints to enhance high-resolution reconstruction quality by more than 2dB PSNR (validated at native resolution).

- ### Connector Module
	Facilitates dynamic alignment of features between frozen MLLM and trainable Diffusion models, achieves semantic alignment for text-to-pixel generation while also ensuring local-global coherence in edits.

- ### AGI-Capable System
	Supports complex chained operations, such as "generate castle → add sunset → adjust perspective," with a swift response time of under 1 second (benchmarked with RTX 4090). The system is designed to handle instruction-driven generation-editing and is synchronized with ChatGPT-4o(aligned with the industry milestone of March 2025).


## Why It Matters

Antu's unified architecture overcomes fundamental limitations of conventional approaches:

| Conventional Methods | Antu's Advantages |
|----------------------|------------------|
| **Modular Pipelines**<br>(CLIP/SigLIP + Diffusion Models) | **End-to-End Unified Model**<br>Seamless understanding-generation integration |
| **Discrete Token AR**<br>(Limited visual grounding) | **Continuous Token Space**<br>Native support for fine-grained visual concepts |
| **Fixed-Resolution Processing**<br>(Artifacts in upscaling) | **Multi-Scale Adaptation**<br>Consistent quality across resolutions |
| **Separate Editing Workflows**<br>(Manual alignment required) | **Dialog-Driven Control**<br>Natural language guided pixel-level editing |
| **Understanding Bottlenecks**<br>(Visual-semantic mismatch) | **Joint Representation Learning**<br>Mutually enhanced comprehension and generation |

## Open Collaboration
We're open-sourcing Antu-α to accelerate progress toward AGI, featuring:
�� Full model weights & test code  
�� Modular architecture for easy extension  
�� Comprehensive benchmarks (vs GPT-4V, SDXL, etc.)

*"The simultaneous release of ChatGPT-4's image generation in March 2025 confirms our vision of unified multimodal AI as the next paradigm."*  

## Empowering Multimodal Interaction with Antu


![效果图](./figures/Ming_unify_usecases.png)
**Antu-α** acts as a unified model for multimodal understanding, extending beyond traditional NLP tasks and multimodal comprehension to enable interactive multimodal generation. This includes capabilities such as image generation, image editing, and style transfer.

## Model Structure

![结构图](./figures/Ming_unify_structure.png)

**Antu-α** is a unified multimodal model designed for both image understanding and high-fidelity image generation. It achieves this by compressing image representations into continuous visual tokens, which are processed alongside discrete text tokens using a scaled auto-regressive Transformer. The generation capability is powered by an externally trained diffusion model (SANA), conditioned on tokens produced by the Transformer.
## Example Usage
- ###Dependencies and Installation
#### System Requirements
- **Python:** >= 3.8
- **PyTorch:** >= 2.4.1+cu12.2 (CUDA 12.2 compatible)

#### Installation

To set up the environment, use pip to install the following dependencies:

```bash
pip install torch==2.4.1 torchvision==0.16.2 torchaudio==2.4.0 tensorflow==2.13.1 numpy==1.24.4 pandas==2.0.1 scipy==1.10.1 scikit-learn==1.3.2 h5py==3.10.0 transformers==4.46.3 diffusers==0.33.0 datasets==2.15.0 sentence-transformers==3.2.1 tokenizers==0.20.3 safetensors==0.4.1 accelerate==0.33.0 deepspeed==0.16.0 bitsandbytes==0.39.0 flash-attn==2.6.3 peft==0.12.0
```

- ### Usage Guided
Below is an example of how to load and use the model:
```python
from transformers import AutoModel, AutoTokenizer

Load the model and tokenizer
model_name = "your-username/your-model-name"
tokenizer = AutoTokenizer.from_pretrained(model_name)
model = AutoModel.from_pretrained(model_name)

Example input
image_file = None
prompt = "Produce image: a smiling man with dark hair sits on a wooden bench wearing a black shirt, khaki pants, and a black belt he accessorizes with a silver and white watch"
generate_prefix = "Production done: <image>" 

Process outputs
print(outputs)
```
For more advanced usage, such as fine-tuning or generating images, refer to the documentation.




## Acknowledgments

The project is currently in its early stages. While some preliminary results have been promising, substantial progress is needed to achieve seamless integration of understanding and generation. Both the code and models require further refinement and optimization, which is why we have chosen to open-source the project. We invite contributions from the community to help enhance and develop it collaboratively. If you have any suggestions or identify issues within the code, please contribute via Pull Requests. Thank you for your support and interest!

## Contact Information

Please submit a GitHub issue if you want help or have issues using Ming.

## License

Ming is licensed under [the MIT License](https://github.com/inclusionAI/Ming/blob/master/LICENCE).



==> sections_omni/3_app.tex <==

\section{Application: Natural Multimodal Interaction}

To support alignment and evaluation, both automated and human, and to demonstrate the application-readiness of our approach, we augment the inference strategy with respect to interleaved generation to improve throughput and reduce latency.

Autoregressive, mixed-modal generation introduces unique performance-related challenges at inference time. These include:
\begin{itemize}
    \item \textbf{Data-dependencies per-step} --- given that our decoding formulation changes depending on whether the model is generating images or text at a particular step, tokens must be inspected at each step (i.e. copied from the GPU to the CPU in a blocking fashion) to guide control flow.
    \item \textbf{Masking for modality-constrained generation} --- to facilitate exclusive generation for a particular modality (e.g. image-only generation), tokens that do not fall in a particular modality space must be masked and ignored when de-tokenizing.
    \item \textbf{Fixed-sized text units} --- unlike text-only generation, which is inherently variable-length, token-based image generation produces fixed-size blocks of tokens corresponding to an image.
\end{itemize}

Given these unique challenges, we built a standalone inference pipeline based on PyTorch \citep{pytorch} supported with GPU kernels from \texttt{xformers} \citep{xFormers2022}. 

Our inference implementation supports streaming for both text and images. When generating in a streaming fashion, token-dependent conditional logic is needed at each generation step. Without streaming, however, blocks of image tokens can be generated in a fused fashion without conditional computation. In all cases, token masking removes branching on the GPU. Even in the non-streaming setting, however, while generating text, each output token must be inspected for image-start tokens to condition image-specific decoding augmentations.

\paragraph{\textbf{Chatting}} xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx.

\paragraph{\textbf{Multimodal Chatting}} xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx.

\paragraph{\textbf{Image Generation}} xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx.

\paragraph{\textbf{Image Editing}} xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx.

\paragraph{\textbf{Image Style Transfer}} xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx.

\paragraph{\textbf{Multi-view Generation}} xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 

% \paragraph{\textbf{3D Rendering}} xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx.

% \paragraph{\textbf{Multi-subject Fusion}} xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx.

% \paragraph{\textbf{Customized Image Generation}} xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx.


==> sections_omni/8_future.tex <==

\section{Future Work}
\enlargethispage{2\baselineskip}
This report outlines our technical approach and preliminary results. Further updates will be released soon. Below, we summarize several directions we plan to pursue in the near future:

% 1. 对xxx的多阶段训练过程的详细汇报，包括数据细节，数据配比，损失下降曲线，训练步数，中间结果等，以及更细粒度的定性定量的实验分析
% 2. 扩展更多task的数据，实现更加强大的基于多模态对话的图像生成或编辑


\begin{itemize}
\item \textbf{Experiment}: Provide a detailed report on the multi-stage training process of \model{}, covering data details, data composition ratios, loss curves, training steps, intermediate results, and fine-grained qualitative and quantitative experimental analysis.

\item \textbf{Data}: Expand the post-training dataset to support a wider range of tasks, enabling advanced image generation and editing based on text prompts.

\item \textbf{Architecture}: xxxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx


\item \textbf{Scaling-up}: xxxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx

\end{itemize}


==> sections_omni/dxn_abandon_table.tex <==
% ***--***--*** 1. OC Normal
        \caption{
            Performance of \modellite{} on \textbf{OpenCompass Image-Text Basic Benchmarks} compared to leading MLLMs.
        }
	\small
	\vspace{-0.2cm}
	\centering
        \begin{tabular}{
            p{3.0cm}<{\centering}p{1.8cm}<{\centering}p{1.8cm}<{\centering}p{1.8cm}<{\centering}p{1.8cm}<{\centering}p{1.8cm}<{\centering}p{1.8cm}<{\centering}
        }
            \hline
		\multicolumn{1}{c|}{\multirow{2}{*}{Benchmark}} &
            \multicolumn{1}{c}{\modellinefirst{}} &
		\multicolumn{1}{c}{Ola} &
		\multicolumn{1}{c}{Ovis2} &
		\multicolumn{1}{c}{Qwen2.5VL} &
		\multicolumn{1}{c}{InternVL2.5} &
		\multicolumn{1}{c}{Gemma3}
		\\ 
		\multicolumn{1}{c|}{}&
		\multicolumn{1}{c}{\modellinesecond{}} &
            \multicolumn{1}{c}{7B} &
		\multicolumn{1}{c}{8B} &
		\multicolumn{1}{c}{7B-Instruct} &
		\multicolumn{1}{c}{8B-MPO} &
		\multicolumn{1}{c}{27B}
		\\ \hline
        % \multicolumn{7}{c}{\multirow{1}{*}{ \textit{Methods: Video-text Pre-training from Scratch}}} \\\hline
        \multicolumn{1}{c|}{AI2D} & 83.1 & 86.1 & \underline{\textbf{86.6}} & 84.4 & 84.5 & 81.4
		\\ % \hline
        \multicolumn{1}{c|}{HallusionBench} & 55.0 & 53.5 & \underline{\textbf{56.3}} & 55.8 & 51.7 & 48.8
		\\ % \hline
        \multicolumn{1}{c|}{MMBench-TEST-V11} & 80.8 & \underline{\textbf{84.3}} & 83.6 & 82.8 & 82.0 & 78.9
		\\ % \hline
        \multicolumn{1}{c|}{MMMU} & 56.3 & 57.0 & 57.4 & 56.6 & 54.8 & \underline{\textbf{64.8}}
		\\ % \hline
        \multicolumn{1}{c|}{MMStar} & 64.7 & \underline{\textbf{70.8}} & 64.6 & 65.3 & 65.2 & 59.6
		\\ % \hline
        \multicolumn{1}{c|}{MMVet} & 71.3 & \underline{\textbf{78.6}} & 65.1 & 71.6 & 68.1 & 71.0
		\\ % \hline
        \multicolumn{1}{c|}{MathVista} & 71.6 & 68.4 & \underline{\textbf{71.8}} & 68.1 & 67.9 & 67.6
		\\ % \hline
        \multicolumn{1}{c|}{OCRBench} & 88.4 & 82.2 & \underline{\textbf{89.1}} & 87.8 & 88.2 & 75.3
		\\ \hline
        \multicolumn{1}{c|}{Average} & 71.4 & \underline{\textbf{72.6}} & 71.8 & 71.5 & 70.3 & 68.4
		\\ \hline

        \label{table_1_ocnormal}
	\end{tabular}

        \vspace{-0.2cm}

        % ***--***--*** 2. OC Reasoning
        \caption{
            Performance of \modellite{} on \textbf{OpenCompass Image-Text Reasoning Benchmarks} compared to leading MLLMs. The superscript ``$^{v}$'' denotes benchmarks that are evaluated using vision-only models.
        }
	\small
	\vspace{-0.2cm}
	\centering
        \begin{tabular}{
            p{2.4cm}<{\centering}p{1.6cm}<{\centering}p{1.6cm}<{\centering}p{1.6cm}<{\centering}p{1.6cm}<{\centering}p{1.6cm}<{\centering}p{1.6cm}<{\centering}p{1.4cm}<{\centering}
        }
            \hline
		\multicolumn{1}{c|}{\multirow{2}{*}{Benchmark}} &
            \multicolumn{1}{c}{\modellinefirst{}} &
		\multicolumn{1}{c}{Taichu-VLR} &
		\multicolumn{1}{c}{VLAA} &
		\multicolumn{1}{c}{Gemma3} &
		\multicolumn{1}{c}{InternVL3} &
		\multicolumn{1}{c}{Qwen2.5VL} &
		\multicolumn{1}{c}{Ovis}
		\\ 
		\multicolumn{1}{c|}{} &
		  \multicolumn{1}{c}{\modellinesecond{}} &
            \multicolumn{1}{c}{7B} &
		\multicolumn{1}{c}{Thinker-7B} &
		\multicolumn{1}{c}{27B} &
		\multicolumn{1}{c}{8B} &
		\multicolumn{1}{c}{7B-Instruct} &
		\multicolumn{1}{c}{8B}
		\\ \hline
        % \multicolumn{7}{c}{\multirow{1}{*}{ \textit{Methods: Video-text Pre-training from Scratch}}} \\\hline
        \multicolumn{1}{c|}{MathVista-MINI} & 68.1 & \underline{\textbf{72.3}} & 68.0 & 67.6 & 70.5 & 68.1 & 71.8
		\\ % \hline
        \multicolumn{1}{c|}{DynaMath} & 23.0 & 23.0 & 22.4 & \underline{\textbf{27.5}} & 25.7 & 19.6 & 20.4
		\\ % \hline
        \multicolumn{1}{c|}{LogicVista} & 40.7 & 48.3 & \underline{\textbf{48.5}} & 47.9 & 44.5 & 47.0 & 39.4
		\\ % \hline
        \multicolumn{1}{c|}{MathVerse-MINI$^{v}$} & 35.3 & 46.7 & \underline{\textbf{48.2}} & 31.3 & 38.5 & 39.0 & 42.3
		\\ % \hline
        \multicolumn{1}{c|}{MathVision} & 26.1 & 27.1 & 26.4 & \underline{\textbf{36.7}} & 30.0 & 27.0 & 25.9
		\\ % \hline
        \multicolumn{1}{c|}{WeMath} & 33.2 & \underline{\textbf{44.0}} & 41.5 & 40.7 & 39.5 & 36.2 & 27.2
		\\ % \hline
        \hline
        \multicolumn{1}{c|}{Average} & 37.7 & \underline{\textbf{43.6}} & 42.5 & 42.0 & 41.5 & 39.5 & 37.8
		\\ \hline

        \label{table_2_ocreasoning}
	\end{tabular}

        \vspace{-0.2cm}

        % ***--***--*** 4. Object detection
        \caption{
            Performance of \modellite{} on \textbf{PUBLIC Grounding Benchmarks} compared to leading MLLMs.
        }
	\small
	\vspace{-0.2cm}
	\centering
        \begin{tabular}{
            p{1.8cm}<{\centering}p{1.0cm}<{\centering}|p{2.0cm}<{\centering}p{2.0cm}<{\centering}p{2.0cm}<{\centering}p{2.0cm}<{\centering}p{2.0cm}<{\centering}
        }
            \hline
		\multicolumn{1}{c}{\multirow{2}{*}{Benchmark}} &
            \multicolumn{1}{c|}{\multirow{2}{*}{Split}} &
            \multicolumn{1}{c}{\modellinefirst{}} &
            \multicolumn{1}{c}{Qwen2.5-Omni} &
            \multicolumn{1}{c}{InternVL2.5} &
		\multicolumn{1}{c}{Grounding-DINO} &
		\multicolumn{1}{c}{Qwen2.5VL} 
		\\ 
		&
            &
		\multicolumn{1}{c}{\modellinesecond{}} &
            \multicolumn{1}{c}{7B} &
            \multicolumn{1}{c}{8B} &
            \multicolumn{1}{c}{Large} &
		\multicolumn{1}{c}{7B-Instruct} 
		
		\\ \hline
        % \multicolumn{7}{c}{\multirow{1}{*}{ \textit{Methods: Video-text Pre-training from Scratch}}} \\\hline
        & val & \underline{\textbf{90.6}} & 90.5 & 90.3 & \underline{\textbf{90.6}} & 90.0
		\\ % \hline
        RefCOCO & testA & 93.1 & 93.5 & \underline{\textbf{94.5}} & 93.2 & 92.5
		\\ % \hline
        & testB & 86.3 & 86.6 & 85.9 & \underline{\textbf{88.2}} & 85.4
		\\ \hline
        & val & \underline{\textbf{85.4}} & \underline{\textbf{85.4}} & 85.2 & 82.8 & 84.2
		\\ % \hline
        RefCOCO+ & testA & 89.8 & 91.0 & \underline{\textbf{91.5}} & 89.0 & 89.1
		\\ % \hline
        & testB & 79.2 & \underline{\textbf{79.3}} & 78.8 & 75.9 & 76.9
		\\ \hline
        \multicolumn{1}{c}{\multirow{2}{*}{RefCOCOg}} & val & 86.8 & \underline{\textbf{87.4}} & 86.7 & 86.1 & 87.2
		\\ % \hline
        & test & 87.5 & \underline{\textbf{87.9}} & 87.6 & 87.0 & 87.2
		\\ % \hline
        \hline
        \multicolumn{2}{c|}{Average} & 87.3 & \underline{\textbf{87.7}} & 87.6 & 86.6 & 86.6
		\\ \hline

        \label{table_4_ocobjdet}
	\end{tabular}

        \vspace{-0.2cm}



% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------



 % ***--***--*** 1. OC Normal
        \caption{
            Performance of \modellite{} on \textbf{OpenCompass Image-Text Benchmarks} compared to leading MLLMs.
        }
	\small
	\vspace{-0.2cm}
	\centering
        \begin{tabular}{
            p{3.0cm}<{\centering}p{1.8cm}<{\centering}p{1.8cm}<{\centering}p{1.8cm}<{\centering}p{1.8cm}<{\centering}p{1.8cm}<{\centering}
        }
            \hline
		\multicolumn{1}{c|}{\multirow{2}{*}{Benchmark}} &
            \multicolumn{1}{c}{\modellinefirst{}} &
		\multicolumn{1}{c}{Qwen2.5} &
            \multicolumn{1}{c}{Qwen2.5VL} &
		\multicolumn{1}{c}{InternVL2.5} &
		\multicolumn{1}{c}{Gemma3}
		\\ 
		\multicolumn{1}{c|}{}&
		\multicolumn{1}{c}{\modellinesecond{}} &
            \multicolumn{1}{c}{Omni} &
		\multicolumn{1}{c}{7B-Instruct} &
		\multicolumn{1}{c}{8B} &
		\multicolumn{1}{c}{27B}
		\\ \hline
        % \multicolumn{7}{c}{\multirow{1}{*}{ \textit{Methods: Video-text Pre-training from Scratch}}} \\\hline
        \multicolumn{1}{c|}{AI2D} & 83.1 & 83.2 & 84.4 & 84.5 & 81.4
		\\ % \hline
        \multicolumn{1}{c|}{HallusionBench} & 55.0 & - & 55.8 & 51.7 & 48.8
		\\ % \hline
        \multicolumn{1}{c|}{MMBench-TEST-V11} & 80.8 & 81.8 & 82.8 & 82.0 & 78.9
		\\ % \hline
        \multicolumn{1}{c|}{MMMU} & 56.3 & 59.2 & 56.6 & 54.8 & \underline{\textbf{64.8}}
		\\ % \hline
        \multicolumn{1}{c|}{MMStar} & 64.7 & 64.0 & 65.3 & 65.2 & 59.6
		\\ % \hline
        \multicolumn{1}{c|}{MMVet} & 71.3 & 66.8 & 71.6 & 68.1 & 71.0
		\\ % \hline
        \multicolumn{1}{c|}{MathVista} & 71.6 & 67.9 & 68.1 & 67.9 & 67.6
		\\ % \hline
        \multicolumn{1}{c|}{OCRBench} & 88.4 & 57.8 & 87.8 & 88.2 & 75.3
		\\ \hline

        % OC
        % \multicolumn{7}{c}{\multirow{1}{*}{ \textit{Methods: Video-text Pre-training from Scratch}}} \\\hline
        \multicolumn{1}{c|}{MathVista-MINI} & 68.1 & 67.9 & 68.1 & 67.6 & 70.5 
		\\ % \hline
        \multicolumn{1}{c|}{DynaMath} & 23.0 & - & 19.6 & \underline{\textbf{27.5}} & 25.7 
		\\ % \hline
        \multicolumn{1}{c|}{LogicVista} & 40.7 & - & 47.0 & 47.9 & 44.5
		\\ % \hline
        \multicolumn{1}{c|}{MathVerse-MINI$^{v}$} & 35.3 & - & 39.0 & 31.3 & 38.5 
		\\ % \hline
        \multicolumn{1}{c|}{MathVision} & 26.1 & 25.0 & 27.0 & \underline{\textbf{36.7}} & 30.0 
		\\ % \hline
        \multicolumn{1}{c|}{WeMath} & 33.2 & - & 36.2 & 40.7 & 39.5 
		\\ % \hline
        \hline

        \label{table_2_ocreasoning}
	\end{tabular}

        \vspace{-0.2cm}





% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------
% ---------












\begin{minipage}[t]{0.46\linewidth}

        % ***--***--*** 3. OC OCR
        \captionsetup{font={small}}
        \caption{
            Performance of \modellite{} on \textbf{PUBLIC OCR Benchmarks} compared to leading MLLMs.
        }
        \small
	\vspace{-0.2cm}
	\centering
        \setlength\tabcolsep{0.1pt}%
        \begin{tabular}{
            p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}
        }
            \hline
		\multicolumn{1}{c|}{\multirow{2}{*}{Benchmark}} &
            \multicolumn{1}{c}{\modellinefirst{}} &
            \multicolumn{1}{c}{InternVL3} &
            \multicolumn{1}{c}{Gemma3} &
		\multicolumn{1}{c}{Qwen2.5VL}
		\\ 
            \multicolumn{1}{c|}{} &
		\multicolumn{1}{c}{\modellinesecond{}} &
            \multicolumn{1}{c}{8B} &
            \multicolumn{1}{c}{27B} &
		\multicolumn{1}{c}{7B-Instruct}
		\\ \hline
        % \multicolumn{7}{c}{\multirow{1}{*}{ \textit{Methods: Video-text Pre-training from Scratch}}} \\\hline
        \multicolumn{1}{c|}{ChartQA} & 85.1 & 86.6 & 83.4 & \underline{\textbf{87.2}}
		\\ % \hline
        \multicolumn{1}{c|}{DocVQA} & 93.0 & 92.7 & 89.5 & \underline{\textbf{95.6}}
		\\ % \hline
        \multicolumn{1}{c|}{OCRBench-v2} & 53.3/52.0 & - & - & \underline{\textbf{56.3}}/\underline{\textbf{57.2}}
		\\ % \hline
        \multicolumn{1}{c|}{TextVQA} & 82.8 & 80.2 & 83.2 & \underline{\textbf{85.1}}
            \\ % \hline
        \multicolumn{1}{c|}{OmniDocBench$\downarrow$} & 34.0/\underline{\textbf{34.4}} & - & - & \underline{\textbf{30.8}}/39.8
		\\ \hline
  %       \multicolumn{1}{c|}{Average} & \underline{\textbf{75.9}} & 74.5
		% \\ \hline

        \label{table_3_ococr}
	\end{tabular}

        \vspace{-0.2cm}

        % ***--***--*** 3. OC GUI
        \captionsetup{font={small}}
        \caption{
            Performance of \modellite{} on \textbf{PUBLIC GUI Benchmarks} compared to leading MLLMs. The superscript ``$^{*}$'' denotes the reproduced results.
        }
        \small
	\vspace{-0.2cm}
	\centering
        \begin{tabular}{
            p{2.0cm}<{\centering}p{1.4cm}<{\centering}p{1.4cm}<{\centering}p{1.6cm}<{\centering}
        }
            \hline
		\multicolumn{1}{c|}{\multirow{2}{*}{Benchmark}} &
            \multicolumn{1}{c}{\modellinefirst{}} &
            \multicolumn{1}{c}{InternVL3} &
		\multicolumn{1}{c}{Qwen2.5VL}
		\\ 
            \multicolumn{1}{c|}{} &
		\multicolumn{1}{c}{\modellinesecond{}} &
            \multicolumn{1}{c}{8B} &
		\multicolumn{1}{c}{7B-Instruct}
		\\ \hline
        % \multicolumn{7}{c}{\multirow{1}{*}{ \textit{Methods: Video-text Pre-training from Scratch}}} \\\hline
        \multicolumn{1}{c|}{ScreenSpot} & \underline{\textbf{82.1}} & 79.5 & 78.9$^{*}$
		\\ % \hline
        \multicolumn{1}{c|}{ScreenSpot-V2} & \underline{\textbf{84.1}} & 81.4 & -
		\\ % \hline
        \multicolumn{1}{c|}{AITZ(EM)} & \underline{\textbf{66.6}} & - & 57.6$^{*}$
		\\ % \hline
        \hline
  %       \multicolumn{1}{c|}{Average} & \underline{\textbf{82.1}} & & 78.9$^{*}$
		% \\ \hline

        \label{table_3_ocgui}
	\end{tabular}

    % ***--***--*** 

    \end{minipage}
\begin{minipage}[t]{0.04\linewidth}
\begin{tabular}{
        p{0.2cm}<{\centering}p{0.2cm}<{\centering}
    }
     &  
\end{tabular}
\end{minipage}
\begin{minipage}[t]{0.50\linewidth}

        % ***--***--*** 7. knowledge
        \captionsetup{font={small}}
        \caption{
            Performance of \modellite{} on \textbf{PUBLIC  Information-Seeking Benchmarks} compared to leading MLLMs.
        }
        \small
	\vspace{-0.2cm}
	\centering
        \begin{tabular}{
            p{2.2cm}<{\centering}p{1.6cm}<{\centering}p{1.0cm}<{\centering}p{1.6cm}<{\centering}
        }
            \hline
		\multicolumn{1}{c|}{Benchmark} &
            \multicolumn{1}{c}{\modellinefirst{}} &
		\multicolumn{1}{c}{PaLI-X} &
		\multicolumn{1}{c}{Qwen2.5VL}
		\\ 
		\multicolumn{1}{c|}{(InfoSeek)} &
		\multicolumn{1}{c}{\modellinesecond{}} &
		\multicolumn{1}{c}{} &
            \multicolumn{1}{c}{32B}
		\\ \hline
        % \multicolumn{7}{c}{\multirow{1}{*}{ \textit{Methods: Video-text Pre-training from Scratch}}} \\\hline
        \multicolumn{1}{c|}{H-mean} & \underline{\textbf{27.7}} & 22.1 & 19.4
		\\ % \hline
        \multicolumn{1}{c|}{Unseen-question} & \underline{\textbf{30.4}} & 23.5 & 20.6
		\\ % \hline
        \multicolumn{1}{c|}{Unseen-entity} & \underline{\textbf{25.4}} & 20.8 & 18.3
		\\ % \hline
        \hline
        
        \label{table_7_knowledge}
	\end{tabular}

        \vspace{-0.2cm}

        % ***--***--*** 6. eyes
        \captionsetup{font={small}}
        \caption{
            Performance of \modellite{} on \textbf{IN-HOUSE Encyclopedia Benchmarks} compared to leading MLLMs.
        }
        \small
	\vspace{-0.2cm}
	\centering
        \begin{tabular}{
            p{1.6cm}<{\centering}p{1.4cm}<{\centering}p{1.6cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}
        }
            \hline
		\multicolumn{1}{c|}{Benchmark} &
            \multicolumn{1}{c}{\modellinefirst{}} &
		\multicolumn{1}{c}{Qwen2.5VL} &
		\multicolumn{1}{c}{Ovis2} &
		\multicolumn{1}{c}{Ola}
		\\ 
		\multicolumn{1}{c|}{(In-house)} &
		\multicolumn{1}{c}{\modellinesecond{}} &
            \multicolumn{1}{c}{7B-Instruct} &
            \multicolumn{1}{c}{8B} &
            \multicolumn{1}{c}{7B}
		\\ \hline
        % \multicolumn{7}{c}{\multirow{1}{*}{ \textit{Methods: Video-text Pre-training from Scratch}}} \\\hline
        \multicolumn{1}{c|}{Plant} & \underline{\textbf{54.96}} & 47.85 & 37.83 & 36.33
		\\ % \hline
        \multicolumn{1}{c|}{Animal} & \underline{\textbf{56.70}} & 50.85 & 45.49 & 40.38
		\\ % \hline
        \multicolumn{1}{c|}{Vehicle} & 41.91 & 42.29 & \underline{\textbf{46.01}} & 39.05
		\\ % \hline
        \multicolumn{1}{c|}{Ingredient} & \underline{\textbf{62.28}} & 54.09 & 54.72 & 53.88
		\\ % \hline
        \multicolumn{1}{c|}{Dish} & \underline{\textbf{44.30}} & 39.07 & 42.56 & 42.56
		\\ % \hline
        \hline
        \multicolumn{1}{c|}{Average} & \underline{\textbf{52.03}} & 46.83 & 45.32 & 42.44
		\\ \hline
        \label{table_6_eyes}
	\end{tabular}

    \end{minipage}
